A New Approach to Voice Authenticity

Voice faking, driven primarily by recent advances in text-to-speech (TTS) synthesis technology, poses significant societal challenges. Currently, the prevailing assumption is that unaltered human speech can be considered genuine, while fake speech comes from TTS synthesis. We argue that this binary distinction is oversimplified. For instance, altered playback speeds can be used for malicious purposes, like in the 'Drunken Nancy Pelosi' incident. Similarly, editing of audio clips can be done ethically, e.g., for brevity or summarization in news reporting or podcasts, but editing can also create misleading narratives. In this paper, we propose a conceptual shift away from the binary paradigm of audio being either 'fake' or 'real'. Instead, our focus is on pinpointing 'voice edits', which encompass traditional modifications like filters and cuts, as well as TTS synthesis and VC systems. We delineate 6 categories and curate a new challenge dataset rooted in the M-AILABS corpus, for which we present baseline detection systems. And most importantly, we argue that merely categorizing audio as fake or real is a dangerous over-simplification that will fail to move the field of speech technology forward.

==> tables/Dataset_Distribution.tex <==
\begin{tabular}{lr}
\toprule
{} &  Proportion \\
\midrule
\textbf{Original Voice \id{human_speech}      } &       34.3\% \\
\textbf{Voice Conversion  \id{vc}    } &        0.0\% \\
\textbf{Voice Cloning  \id{tts_cloning}       } &        0.0\% \\
\textbf{TTS          \id{tts}         } &        0.0\% \\
\textbf{Cut Out \id{trimming}        } &        0.1\% \\
\textbf{Pitch Up \id{inc_pitch}      } &        6.5\% \\
\textbf{Pitch Down \id{dec_pitch}            } &        5.4\% \\
\textbf{Speed Slower \id{slow_speed}        } &       12.0\% \\
\textbf{Speed Faster \id{inc_speed}         } &       12.6\% \\
\textbf{Alaw Encoding \id{alaw}} &       11.8\% \\
\textbf{Ulaw Encoding \id{mlaw}} &       11.3\% \\
\textbf{Added Background Noise ~\id{background_noise}} &        6.0\% \\
\bottomrule
\end{tabular}


==> tables/FC_PerClass.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Accuracy &  F1 Score &    EER \\
\midrule
\textbf{Original Voice        } &     75.8\% &      4.9\% &  45.4\% \\
\textbf{Speed Slower          } &    100.0\% &       NaN & 100.0\% \\
\textbf{Speed Faster          } &     84.8\% &      0.0\% &  41.1\% \\
\textbf{Pitch Up              } &     93.9\% &      7.2\% &  48.5\% \\
\textbf{Pitch Down            } &     95.2\% &      0.0\% &  31.1\% \\
\textbf{Cut Out               } &     34.8\% &     49.6\% &  44.0\% \\
\textbf{Added Background Noise} &     94.7\% &     20.3\% &  36.4\% \\
\textbf{Alaw Encoding         } &     95.5\% &      0.0\% &  51.6\% \\
\textbf{Ulaw Encoding         } &     92.8\% &      0.0\% &  49.1\% \\
\textbf{Voice Conversion      } &    100.0\% &       NaN & 100.0\% \\
\textbf{Voice Cloning         } &    100.0\% &       NaN & 100.0\% \\
\textbf{TTS                   } &    100.0\% &       NaN & 100.0\% \\
\textbf{Overall               } &     33.7\% &     33.7\% &  62.3\% \\
\bottomrule
\end{tabular}


==> tables/LCNNWang_PerClass.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Accuracy &  F1 Score &     EER \\
\midrule
\textbf{Original Voice \id{human_speech}            } &    84.4\% &    71.8\% &  15.1\% \\
\textbf{Voice Conversion \id{vc}                    } &   100.0\% &       NaN & 100.0\% \\
\textbf{Voice Cloning \id{tts_cloning}              } &   100.0\% &       NaN & 100.0\% \\
\textbf{TTS \id{tts}                                } &   100.0\% &       NaN & 100.0\% \\
\textbf{Cut Out \id{trimming}                       } &    91.3\% &    80.6\% &  11.2\% \\
\textbf{Pitch Up \id{inc_pitch}                     } &    97.4\% &    72.2\% &  10.9\% \\
\textbf{Pitch Down \id{dec_pitch}                   } &    99.7\% &    97.3\% &   1.4\% \\
\textbf{Speed Slower \id{slow_speed}                } &    93.0\% &    68.0\% &  12.4\% \\
\textbf{Speed Faster \id{inc_speed}                 } &    93.7\% &    47.3\% &  19.5\% \\
\textbf{Alaw Encoding \id{alaw}                     } &    91.2\% &    62.1\% &  11.2\% \\
\textbf{Ulaw Encoding \id{mlaw}                     } &    92.0\% &    48.1\% &   9.3\% \\
\textbf{Added Background Noise \id{background_noise}} &    99.0\% &    83.5\% &   4.4\% \\
\textbf{Overall                                     } &    70.8\% &    70.8\% &  32.9\% \\
\bottomrule
\end{tabular}


==> tables/Overall_Comparison.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Accuracy &  F1 Score &   EER \\
\midrule
\textbf{FC      } &     33.7\% &     33.7\% & 62.3\% \\
\textbf{LCNNWang} &     74.3\% &     74.3\% &  0.0\% \\
\bottomrule
\end{tabular}


==> tables/results.tex <==
\begin{tabular}{llll|lll|lll|l}
\toprule
Model Name &                    ComplexNet &                     &                     &                          LCNN &                           &         &                     RawNet2 &                      &                       &                      SSL W2V2 \\
Input Length                                    &                          0.35s &                           1.2s &                          4.05s &                          0.35s &                           1.2s &        4.05s &                        0.35s &                         1.2s &                         4.05s &                          4.05s \\
\midrule
Epoch Time (min)                                   &                       4.4±0.2 &                       5.6±0.1 &                      16.1±0.1 &                       4.5±1.0 &                       4.6±0.2 &     8.0±0.2 &                     2.2±0.2 &                     3.0±0.4 &                      5.3±0.9 &                      35.0±0.1 \\
Test Accuracy                                      &                     46.1±11.5 &   \cellcolor{color2} 68.6±9.9 &                      74.3±3.7 &   \cellcolor{color1} 55.6±0.5 &                      63.8±7.0 &    63.6±7.6 &                    11.6±1.5 &                    48.4±8.7 &                     60.8±1.6 &   \cellcolor{color3} 78.6±1.9 \\
\midrule
\textbf{F1 Scores} &&&&&& \\
Original Voice \id{original_voice}                 &                       4.5±0.9 &  \cellcolor{color2} 18.1±25.6 &   \cellcolor{color3} 40.6±5.0 &  \cellcolor{color1} 14.3±13.3 &                      15.7±5.5 &   13.1±18.5 &                     0.0±0.0 &                     0.0±0.0 &                      8.9±4.1 &                     38.6±17.1 \\
Text To Speech \id{text_to_speech}                 &                      31.5±3.5 &                     71.1±22.7 &                     83.1±11.1 &  \cellcolor{color1} 58.2±24.1 &   \cellcolor{color2} 76.3±4.7 &    79.4±9.5 &                     0.0±0.0 &                   48.0±14.2 &                     79.8±5.8 &   \cellcolor{color3} 97.8±0.5 \\
Insert Or Cut Audio \id{insert_or_cut_audio}       &    \cellcolor{color1} 0.0±0.0 &                       4.3±2.3 &                     15.5±10.4 &    \cellcolor{color1} 0.0±0.0 &                       4.1±0.4 &     5.2±7.3 &  \cellcolor{color1} 0.0±0.0 &  \cellcolor{color2} 9.4±7.8 &                      6.7±9.4 &   \cellcolor{color3} 93.2±2.0 \\
Mixing \id{mixing}                                 &                      11.8±0.7 &  \cellcolor{color2} 71.2±11.0 &                      89.0±4.6 &   \cellcolor{color1} 23.0±0.9 &                     47.3±11.7 &    61.7±0.3 &                     0.0±0.0 &                    38.8±4.8 &                    75.6±13.3 &   \cellcolor{color3} 98.3±0.4 \\
Pitch Up \id{pitch_up}                             &   \cellcolor{color1} 76.8±9.9 &   \cellcolor{color2} 91.5±8.1 &                      95.5±1.5 &                     62.9±28.1 &                      84.5±6.2 &    91.7±7.3 &                     0.0±0.0 &                    67.1±9.9 &                     88.0±1.0 &   \cellcolor{color3} 98.2±0.4 \\
Pitch Down \id{pitch_down}                         &                      76.9±7.3 &                      93.7±8.5 &   \cellcolor{color3} 98.6±0.2 &   \cellcolor{color1} 89.1±3.7 &   \cellcolor{color2} 95.7±2.2 &    95.6±5.8 &                     2.4±3.3 &                    77.0±4.3 &                     88.6±1.0 &   \cellcolor{color3} 99.0±0.6 \\
Speed Slower \id{speed_slower}                     &                     46.8±35.6 &  \cellcolor{color2} 75.1±12.6 &                      58.8±5.8 &  \cellcolor{color1} 47.5±12.5 &                     25.0±26.8 &   54.4±11.1 &                     0.0±0.0 &                   23.3±23.1 &                     60.4±1.3 &   \cellcolor{color3} 83.0±3.1 \\
Speed Faster \id{speed_faster}                     &  \cellcolor{color1} 69.6±12.0 &  \cellcolor{color2} 71.0±18.6 &                     41.9±16.8 &                      61.3±1.2 &                      66.1±3.8 &   16.1±14.8 &                    8.6±12.1 &                   48.3±20.7 &                    28.9±23.4 &   \cellcolor{color3} 83.1±3.2 \\
Mp3 Compression \id{mp3_compression}               &                     34.1±39.5 &                     80.3±17.3 &   \cellcolor{color3} 90.6±9.1 &   \cellcolor{color1} 84.9±4.8 &   \cellcolor{color2} 93.6±6.9 &   88.0±15.8 &                     0.0±0.0 &                    10.9±4.5 &                    51.6±16.8 &                      71.4±2.2 \\
Aac Compression \id{aac_compression}               &                      87.4±5.0 &   \cellcolor{color2} 84.8±6.1 &                     78.4±13.4 &   \cellcolor{color1} 88.9±1.5 &                      82.2±6.1 &   30.4±30.0 &                     6.7±9.5 &                    83.8±0.7 &                     68.2±0.3 &   \cellcolor{color3} 79.4±3.6 \\
Alaw Encoding \id{alaw_encoding}                   &                     21.7±27.5 &  \cellcolor{color2} 46.0±15.9 &   \cellcolor{color3} 59.5±4.9 &  \cellcolor{color1} 39.8±17.1 &                      14.0±4.6 &   48.0±22.6 &                     2.1±2.9 &                    7.1±10.1 &                     19.2±9.6 &                       7.3±2.1 \\
Ulaw Encoding \id{ulaw_encoding}                   &                       5.1±7.3 &                      7.9±11.2 &                     10.6±10.8 &  \cellcolor{color1} 26.7±26.1 &  \cellcolor{color2} 42.3±21.3 &    43.7±2.5 &                     0.0±0.0 &                    15.9±4.9 &                      2.0±2.8 &  \cellcolor{color3} 53.7±19.4 \\
High Pass Filter \id{high_pass_filter}             &                      85.1±2.9 &   \cellcolor{color2} 94.7±0.5 &   \cellcolor{color3} 97.1±0.8 &   \cellcolor{color1} 88.0±2.5 &                      92.8±1.2 &    89.0±4.8 &                    16.1±4.4 &                   83.4±11.2 &                     91.8±2.6 &   \cellcolor{color3} 96.3±0.5 \\
Low Pass Filter \id{low_pass_filter}               &                      19.2±7.3 &                     46.0±30.4 &  \cellcolor{color3} 61.9±19.1 &   \cellcolor{color1} 61.2±1.8 &  \cellcolor{color2} 62.9±17.5 &   48.5±45.7 &                     0.0±0.0 &                   13.5±19.1 &                    10.7±13.7 &                      40.5±2.9 \\
Equalization \id{equalization}                     &                      7.3±10.3 &                      18.7±7.5 &                       0.0±0.0 &   \cellcolor{color1} 21.2±6.4 &   \cellcolor{color2} 32.1±8.5 &   15.5±10.3 &                     4.6±6.5 &                     4.6±1.0 &  \cellcolor{color3} 17.8±7.3 &                       5.5±7.8 \\
Auto Tune \id{auto_tune}                           &                     32.3±18.0 &   \cellcolor{color2} 82.8±4.5 &                      93.9±3.9 &   \cellcolor{color1} 45.0±4.9 &                      70.9±7.1 &    73.8±8.4 &                     1.6±2.3 &                   46.5±21.9 &                     69.7±1.2 &   \cellcolor{color3} 98.0±0.0 \\
Room Impulse \id{room_impulse}                     &   \cellcolor{color1} 91.2±2.7 &   \cellcolor{color2} 97.3±0.7 &                      98.1±0.7 &                      83.3±1.0 &                     78.5±11.5 &   70.9±32.1 &                    44.4±6.7 &                    88.0±5.6 &                     95.3±0.5 &   \cellcolor{color3} 99.5±0.4 \\
Reverb \id{reverb}                                 &  \cellcolor{color1} 63.6±17.6 &   \cellcolor{color2} 96.3±1.3 &   \cellcolor{color3} 99.2±0.0 &                      47.3±2.7 &                     77.1±15.0 &   84.2±12.7 &                     3.4±4.8 &                    75.8±9.4 &                     92.6±2.5 &   \cellcolor{color3} 99.9±0.2 \\
Overlay Background Noise \id{overlay_background} &                      74.4±4.4 &   \cellcolor{color2} 96.6±0.1 &   \cellcolor{color3} 98.8±0.4 &   \cellcolor{color1} 78.1±3.9 &                      91.4±1.5 &    91.1±1.0 &                     4.9±6.9 &                    84.1±5.5 &                     95.4±1.7 &   \cellcolor{color3} 98.3±1.2 \\
Noise Reduce \id{noise_reduce}                     &                     42.5±12.0 &   \cellcolor{color2} 88.0±0.0 &   \cellcolor{color3} 99.9±0.2 &   \cellcolor{color1} 57.0±3.2 &                      62.9±4.2 &    94.0±6.7 &                     0.9±1.2 &                   60.3±33.7 &                    91.8±10.1 &   \cellcolor{color3} 99.5±0.3 \\
\bottomrule
\end{tabular}
